The RGB-D Triathlon: Towards Agile Visual Toolboxes for Robots

Deep networks have brought significant advances in robot perception, enabling to improve the capabilities of robots in several visual tasks, ranging from object detection and recognition to pose estimation, semantic scene segmentation and many others. Still, most approaches typically address visual tasks in isolation, resulting in overspecialized models which achieve strong performances in specific applications but work poorly in other (often related) tasks. This is clearly sub-optimal for a robot which is often required to perform simultaneously multiple visual recognition tasks in order to properly act and interact with the environment. This problem is exacerbated by the limited computational and memory resources typically available onboard to a robotic platform. The problem of learning flexible models which can handle multiple tasks in a lightweight manner has recently gained attention in the computer vision community and benchmarks supporting this research have been proposed. In this work we study this problem in the robot vision context, proposing a new benchmark, the RGB-D Triathlon, and evaluating state of the art algorithms in this novel challenging scenario. We also define a new evaluation protocol, better suited to the robot vision setting. Results shed light on the strengths and weaknesses of existing approaches and on open issues, suggesting directions for future research.

==> removing-IL/challenge.tex <==
\label{sec:challenge}

%%%%%%% dataset images %%%%%% 
\begin{figure*} 
    \centering
  \subfloat[RGBD Object dataset \cite{rod}]{%
       \includegraphics[width=0.32\linewidth]{images/rod.pdf}}
    \hfill
  \subfloat[NYU Depth V2 \cite{nyu}]{%
        \includegraphics[width=0.32\linewidth]{images/nyu.pdf}}
    \hfill
  \subfloat[{LineMOD} \cite{linemod}]{%
        \includegraphics[width=0.32\linewidth]{images/linemod.pdf}}
    \hfill
  \caption{Images taken from the datasets. For each dataset, the top row reports the RGB images, and the bottom row reports depth images colored with the Surface method \cite{aakerberg2017depth}.}
  \label{fig:datasets} 
\end{figure*}

%\massi{TASK CHOSEN and MOTIVATIONS}
%\massi{DATASET DESCRIPTIONS (brief, just for the setting)}
As stated above, the aim of this work is to foster research in developing robot systems which are able to perform several visual tasks by applying \taskabbrv methodologies. This is crucial for many reasons. First, the memory resources typically available in a robotic platform are limited, thus it is practically infeasible to store a new deep network for each novel visual task a robot is asked to solve. Second, we may be interested in extending the visual capabilities of an existing robotic system, in order to solve new tasks not considered at the initial stage of deployment. % this is reasonable, especially if data for the new tasks were not available and/or the need for the new task was not forecasted in the initial stage. 
%Obviously, the drawback of producing such visual toolbox might be on the performances, which could not match what we obtain from a task-specific architecture.
In a nutshell, \taskabbrv techniques aim to learn a set of classification/regression models for multiple tasks sequentially. The challenge is to keep the number of task-specific parameters as low as possible while maximizing performance.

{Formally, the \taskabbrv task is defined as follows. Suppose we have a pretrained mdeep model, with parameters $\theta_0$ and a set $\mathcal{T}=\{\mathcal{T}_1,\cdots,\mathcal{T}_N\}$ of $N$ tasks. For each task we have an input space $\mathcal{X}_t\subset \Re^{H\times W \times C}$, with $C$ depending on the input modality (\ie 1 for depth maps, 3 for RGB images and 4 for RGB-D), a feature space $\mathcal{Z}_t$ and an output space $\mathcal{Y}_t$. For simplicity, let us define as $\phi_{\Theta_t}:\mathcal{X}\rightarrow\mathcal{Z}_t$ a task-specific mapping from the input space to the feature space $\mathcal{Z}_t$. The mapping is parametrized by the set $\Theta_t=\{\theta_0; \ \theta_t\}$ which comprises the shared ($\theta_0$) and task-specific parameters ($\theta_t$). Moreover, let us denote as $\psi_{\Omega_t}:\mathcal{Z}_t\rightarrow\mathcal{Y}_t$ the function mapping the feature space to the task-specific output space, parametrized by $\Omega_t$. In our case, $\Omega_t$ are just the weights of the output layer of our neural network. %denoted as $\omega_0$ and $\omega_t$ respectively.
Finally, let us define the mapping from the input to the output space $\Phi_{t}:\mathcal{X}\rightarrow\mathcal{Y}_t$, where $\Phi_t=\psi_t \circ \phi_{\Theta_t}$. %$\Theta_t=\{\omega_0;\omega_t\}$, is the union of both shared and task-specific parameters denoted as $\omega_0$ and $\omega_t$ respectively. 
We also denote as $\rho_t=|\theta_t|$, the memory size (in bits) required to store the task-specific parameters $\in \Theta_t$ and as $\alpha_t$ a task-specific performance measure (\eg classification accuracy). %in bit of the task specific parameters introduced to map an image int%The goal of a model $\mathcal{M}$ applied to this task is to obtain a set of parameters $\Omega^\mathcal{M}=\{\omega_1^\mathcal{M},\cdots, \omega_N^\mathcal{M}\}$ where $\omega_i^\mathcal{M}$ denotes the parameters learned to address the %is to train, for the task $\mathcal{T}_i$ a set of task-specific parameters $\omega_i^m$ which maximize the performances of the model $a_i^{m}$. As baselines, we denote %with $a_i^{m}$ the performance of model $m$ on task $\mathcal{T}_i$,
%by $a^e_i$ the performances of the feature extractor baseline (\ie the network is frozen, just the output layer is trained for each task) and by $a^f_i$ the performances of the fine-tuned model (\ie all the parameters of the network are copied and fine-tuned for each new task) model. We highlight that the performance metric $a_i^m$ is specific to the task $i$. Similarly, we denote as $p^m_i=|\omega^m_i|$ the size (in bit) of the additional parameters required by the network to perform task $i$, with $p_0=|\omega_0|$ denoting the size of the parameters shared by all tasks. The size computed by $|\omega|$ consider all the weights of the layers with parameters (\eg convolutional, fully-connected) and \textit{do not} consider the components strictly needed to perform a task (\ie the output layers), following \cite{rebuffi_1}.
The goal of an \taskabbrv algorithm is to learn a set of task-specific mappings $\Phi_t$ while i) maximizing $\alpha_t$ and ii) keeping $\rho_t$ as low as possible for any $t \in \mathcal{T}$.
%\begin{itemize}
   % \item Learn multiple task sequentially, without losing performances on old tasks while learning new task-specific models.
    %\item It should keep the number of task-specific parameters $\omega_t^\mathcal{M}$ within as low as possible.
    %\item It should allow to learn a task-specific mapping $\Phi_t^\mathcal{M}$ whose performances $\alpha_t^\mathcal{M}$ are as close as possible to a deep architecture derived by fine-tuning a pre-trained model on each task.
%\end{itemize}
%Based on the above considerations, an effective \taskabbrv approach should have the following properties:
%\begin{itemize}
 %   \item It should permit to learn multiple task sequentially, without losing performances on old tasks while learning new task-specific models.
  %  \item It should keep the number of task-specific parameters as low as possible.
   % \item It should allow to build task-specific models which achieve performances as close as possible to deep architectures derived by fine-tuning a pre-trained model on each task.
%\end{itemize}

To stimulate the research community in robot vision on \taskabbrv, in this paper we propose a dataset consisting in three different tasks and introduce an evaluation metric suitable to the STML setting. The dataset is a collection of three datasets commonly used in the robotic community, but in this paper we propose their joint adoption for studying the novel problem of \taskabbrv.}

In the following subsections, we present the dataset and the tasks we proposed. Then, we describe the novel evaluation protocol we introduced for \taskabbrv in robotics.

\subsection{The \challenge \hspace{2pt}Dataset}
\label{tasks}
The proposed dataset considers three fundamental tasks: object recognition, pose estimation and scene classification. In choosing the tasks and benchmarks we follow three principles, namely i) the importance of the perception task for robotics; ii) the impact that the dataset has had in the past within the community; iii) the possibility of defining a standard training/testing protocol. Differently from challenges in computer vision \cite{rebuffi_1}, we propose three different settings: i) use only RGB images, ii) use only depth images, iii) use both RGB and depth images. Each setting is independent from the others, such as to permit to the researchers to work only on the setting which is more relevant to their application. %\massi{Figure \ref{fig:datasets} show an examples of the images of each dataset and how their depth images have been transformed for training (Section \ref{sec:experiments}).}  % one they want to attack.



\myparagraph{Task 1. Object Recognition.}
%The most basic recognition task a visual system should be capable to perform is
Object recognition is of utmost importance in robotic perception. 
This task consists in assigning to an input image depicting an object the corresponding semantic class label. Object recognition algorithms are fundamental tools for robots because i) knowing the category of an object allows reasoning on how the object can be manipulated and ii) they enable more complex tasks such as object detection. % For this reason, we deincluded this task in our challenge.

We consider the popular RGB-D Object Dataset \cite{rod}. It contains 300 common household objects organized in 51 categories. The dataset was recorded using a Kinect style 3D camera that gathers 30 synchronized and aligned $ 640 \times 480$ RGB and depth images per second. Each object was placed on a turntable during the recording and it was captured during a whole rotation. For each object, there are three video sequences, corresponding to the camera mounted at a different height (so that the object is seen from different angles, \ie approximately 30, 45, and 60 degrees relative to the horizon).
The performance of a model on this task are evaluated as the accuracy on the test samples. We use the same evaluation protocol of %In combination with the dataset, in
\cite{rod} %the authors also proposed an evaluation protocol. The dataset is 
subsampling the dataset by taking every fifth frame, resulting in 41,877 RGB-D images for training and evaluation. They defined 10 pre-defined training and test splits for cross-validation, and in each split, one random object instance from each class is left out from the training set and used for testing. This results in roughly 35,000 training images and 7,000 testing images in each split. At test time, the classifier has to assign the correct label to a previously unseen object instance from each of the 51 classes. For training and test we use the first split among the ten available.%At test time, the classifier has to assign the correct label to a previously unseen object instance from each of the 51 classes. We adopt this setting using the first split among the ten available. %, in order to avoid the need of multiple runs. %training multiple times the multi-task network on different splits of the same dataset. 


%It can be computed using the following formula:
%\begin{gather}
%a_{OR} = \frac{1}{|D_{TEST}|}\sum_{(x_i,y_i) \in D_{TEST}} \boldsymbol{1}( %\phi(x_i) = y_i),
%\end{gather}
%where $D_{TEST}$ is the test dataset, $\phi$ is the neural network function and $\phi(x)$ the predicted class.

\myparagraph{Task 2. 3D Pose Estimation.}
%The second task of our challenge is pose estimation.
Pose estimation refers to the task of predicting the pose of an object with respect to the viewer's camera. This task is important in robotics, \eg due to the information it provides for grasping and manipulating an object \cite{johns2016deep}. The pose estimation task can be decomposed in two sub-tasks: the localization of the object in the image and the estimation of the rotation matrix between the object and the camera. Even though many works attempt to perform both sub-tasks at the same time \cite{bb8,poseCNN}, following \cite{poseregression, learningdescriptors} in this paper we assume that the object is always centered in the input image, reducing the pose estimation task only to the latter sub-task, \ie 3D pose estimation.
%%This is motivated by the fact that object localization is a well-known task in computer vision and can be performed by an object detection system, for which exists many implementations such as \cite{ssd, yolo} that can do it even in real-time.So, for us, the pose estimation task consists in converting an image into a rotation matrix representation, such as the one made by the three angles azimuth, elevation and camera tilt, or axis-angle representation, or quaternions.


We consider the LineMOD dataset \cite{linemod}. We choose this dataset since it is a standard benchmark in robotics and it also provides depth information, as opposed to other benchmarks \cite{xiang2014beyond}. It contains 18000 RGB-D images with 15 different objects classes. We adopt the cropped version of the dataset that was proposed in \cite{learningdescriptors}.
In this version all the images are squared with size $64 \times 64$ pixels and they contain the objects centered in the scene. The ground truth of the pose is given in the form of $3 \times 3$ rotation matrix that maps the camera world coordinate into camera coordinates. 

Some methods tested on this dataset consider the use of both synthetic and real images %, where the synthetic images are generated by the authors and for the real images half are considered for training and the other half as test set \eg 
\cite{zakharov20173d,wohlhart2015learning}. % in order to consider a reproducible experimental setup and avoid arbitrary synthetic data generation procedures, 
In this paper, in order to have a simpler experimental setup, we follow \cite{porzi2017depth} and we consider a setting where only real images are used for training and testing the models. In particular, we use $80\%$ of the images for training and 20$\%$ for testing. % of the The full dataset was split in training and test set by picking one image every five and putting it into the test dataset. The other four images belong to the training set. 

% Penso che la parte a seguire possa essere rimossa o al piu' essere messa come risorsa addizionale
%It provides some advantages: it is a compact representation, using only 4 numbers instead of the 9 parameters of the %rotation matrix, it is numerically stable and avoids the \textit{gimbal lock} phenomenon.
%
%The difference rotation quaternion that represent the difference rotation is defined as $r \doteq pq^*$. The distance %between rotations represented by $p$ and $q$ is the angle of this difference rotation quaternion $r$:
%\begin{gather}
%    cos(\frac{\theta}{2}) = p_1q_1 + p_2q_2 + p_3q_3 + p_4q_4, \\
%    \label{eq:geodesic}
%    \theta = 2 \arccos (| p_1q_1 + p_2q_2 + p_3q_3 + p_4q_4 |).
%\end{gather}
%The equation \ref{eq:geodesic} define the geodesic distance between rotation represented by quaternions. This is the %optimal way to represent the distance in this non-Euclidean space. Other distances, such as the L2 distance (or %Euclidean distance), do not represent well the distance in this space and should be avoided.

For evaluating the performances of a model in the pose estimation task we consider both the prediction of the pose of the object and its semantic class. In particular, we consider a pose to be correctly estimated if the predicted object class is correct and the geodesic error of the predicted rotation is less then 20 degrees. %The first is computed by comparing the predicted label with the ground-truth class, while the latter is evaluated by computing the geodesic distance between the predicted quaternion and the ground-truth rotation represented by a quaternion.
%In particular, we consider a pose to be correctly estimated if the predicted object class is correct and the geodesic error of the predicted rotation is less then 20 degrees.} %the accuracy is computed using the following function:
%\begin{gather}
%	a_{PE} = \frac{1}{m}\sum_{i=1}{m} \boldsymbol{1}( \phi(x_i) = y_i,\: \theta(\psi(x_i), r_i) < 20 ),
%\end{gather}
%where $m$ is the size of the test set, $x_i, y_i, r_i$ are, respectively, the image, the class and the ground truth quaternion of the i-th sample in the test set, $\phi(x_i)$ is the label predicted by the model, $y_i$ is the ground truth label, $\psi(x_i)$ is the quaternion predicted by the model, $r_i$ is the ground truth rotation, and $\theta(\cdot)$ is a function that computes the geodesic distance between quaternions expressed in degrees.


\myparagraph{Task 3. Scene Classification.}
This task consists into assigning to an image a label that indicate the place where the picture was taken. Semantically localizing a robot provides relevant information on how the robot should interact with the environment. %, in particular in terms of the actions it can take.

We use the popular NYU-Depth V2 dataset \cite{nyu}, employed by many previous works \cite{song2017combining,song2017combining,du2018depth}. The dataset contains 1449 pairs of synchronized RGB and depth images, gathered from a wide range of commercial and residential buildings in three different US cities, comprising 464 different indoor scenes across 27 scene classes. Anyway, most of these scene classes are not well represented, thus, following  \cite{Gupta_2013_CVPR}, we reorganized the original 27 categories into 10 classes (\ie the 9 most represented categories and the rest).
The dataset is split in training and test data. Following \cite{nyu} 795 images belong to training data and 654 to the test set. The performance of the model is evaluated as the classification accuracy on test set.


%The accuracy of the model represents the number of correct labels assigned to the examples of the test dataset. It can be computed using the following formula:
%\begin{gather}
%a_{SC} = \frac{1}{|D_{TEST}|}\sum_{(x_i,y_i) \in D_{TEST}} \boldsymbol{1}( \phi(x_i) = y_i),
%\end{gather}
%where $D_{TEST}$ is the test dataset, and $\phi(x)$ the predicted class.




==> removing-IL/conclusions.tex <==
We presented a novel benchmark for robot visual systems, namely the \challenge. This novel setting allows to compare model in the \taskname scenario where, starting from a pre-trained architecture, the goal is to learn diverse visual tasks while obtaining performances as close as possible of a task-specific architecture and keeping as low as possible the number of additional parameters required per-task. We propose a proper metric for this task which takes into accounts both the performances and the number of parameters employed. We then evaluate state-of-the-art sequential multi-task learning methods on this new benchmark and with classical and novel metrics, reporting the needed baselines for researchers interested on tackling this problem. We hope that this benchmark will highlight the need for the development of efficient and effective vision algorithms, which is crucial for robots. While the first setting proposed involves 3 tasks, our definition of the task, metrics and baselines is modular and can be easily extended to include other different tasks.

==> removing-IL/intro.tex <==
Recent years have witnessed great advances in computer and robot vision thanks to deep networks \cite{krizhevsky2012imagenet}. % These networks and their variants achieved very high performances on many tasks but they require millions of parameters and a lot of computations both for training and inference. Often these algorithms are executed by clusters with many GPUs, therefore, with a lot of computational resources, and with terabytes of memory (RAM).
%\textcolor{red}
Deep models are used in many applications in robot vision, ranging from egomotion estimation \cite{costante2016exploring} to depth prediction \cite{jafari2017analyzing,mancini2017toward},
object grasping \cite{johns2016deep, levine2018learning}
semantic segmentation \cite{schwarz2018rgb,oliveira2018efficient}, etc.

A common procedure %when developing a novel deep architecture
for addressing a specific visual recognition problem consists in fine-tuning an existing pretrained model on a given, problem-specific dataset.  
%This imply considering each visual recognition tasks in isolation and overspecializing the network models to the given task. 
While this strategy leads to excellent performance on the specific problem and setting, it ignores two key aspects of robot vision. The first is that robots need visual abilities for several tasks. For instance, to complete a simple carrying task a robot needs to localize itself, detect and recognize the objects in front of it and estimate their poses (see Fig. \ref{fig:teaser}). Clearly, having an overspecialized network for each specific task would scale poorly. Second, the multiple tasks that a robot is required to solve are often closely related (see Fig. \ref{fig:teaser}). Hence, addressing the tasks jointly would probably lead to an increased accuracy as well as to an improved computational efficiency with respect to training task-specific networks.

%Obviously, this is not applicable in the robotic context. Robots must make decisions in real time but they can neither mount a cluster to perform the computation due to both spatial and energy constraints, nor connect to a cluster through the Internet due to the latency that it will generate. Thus, it is necessary to use models with fewer parameters than those used in computer vision.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/Sys1.pdf}
    \caption{The ability of the robot to perform multiple task at the same time is crucial. In this example, a robotic arm should manipulate correctly the object in the scene, thus must understand the class of the object, its orientation and the overall context in which it operates.}
        \label{fig:teaser}
\end{figure}

To deal with this issue, over the years Multi-Task Learning (MTL) \cite{Caruana1997} approaches have been developed. 
MTL refers to jointly learn a set of classification/regression models, each associated to a specific task, by leveraging information about task relatedness, \eg sharing models' parameters. By reducing the number of parameters, MTL %needed by sharing them between different tasks 
also decreases the time needed for model training and inference.
MTL has been successfully applied in robotics: 
%For instance 
Teichmann \etal \cite{teichmann2018multinet} proposed an architecture  performing jointly object detection, classification, and semantic segmentation. Similarly, in \cite{rahmatizadeh2018vision} Rahmatizadeh \etal described a technique to train a controller to perform several complex picking and placing tasks.

\massi{REPLACE
MTL assumes that the data for all the tasks are available during training. In robotics this assumption is often unrealistic and the ability to add new tasks sequentially %to an existing model 
is crucial %in many applications 
\cite{mitchell2018never, thrun1998lifelong}.  However, a well-known problem of  sequential learning is that, while learning how to perform a new task, an algorithm typically forgets about previous tasks. This %phenomenon, referred to as 
\textit{catastrophic forgetting} \cite{catforg_1, catforg_2} must be kept into account while developing visual recognition models. % able to avoid it or limit its effect.



Sequential Multi-Task Learning (SMTL)  algorithms \cite{rebuffi_1, rebuffi_2, packnet, piggyback, quantized} automatically address the catastrophic forgetting problem by considering a common network backbone and introducing a small set of task-specific network parameters. In practice, during training, for each new task these methods instantiate and learn few task-specific parameters (see Fig. \ref{fig:SMTL}),
%add only the extra task-specific parameters are optimized, 
while the other network's weights are kept fixed. While interesting and effective, % to adapt a model to novel tasks, these solutions
these approaches have been considered only in computer vision and it is not clear if they can also be used in a % not respect the constraints of the 
robotic setting where %not only the model accuracy but 
the computational/memory requirements are especially relevant.} 

This paper aims to demonstrate that SMTL can be successfully applied to robotic perception tasks and that it constitutes a better strategy with respect to network fine-tuning and naive classifier learning. In particular, considering a pretrained network architecture and fine-tuning it for each task leads to strong classification performances but this approach is not scalable as it requires the robot to store a whole network for each task. On the other hand, just using a network with fixed weights as feature extractor and training only task-specific output layers is also suboptimal. In fact, while this solution has almost no overhead in terms of parameters, the corresponding models will be less accurate. To study Sequential Multi-Task Learning, in this paper we propose the first SMTL benchmark for robot vision and test state of the art algorithms on this dataset. Moreover, to take into account the peculiarities of the robotics scenario, we propose a new evaluation protocol which allows to compare different SMTL algorithms considering not only their recognition performances but also their memory requirements and their ability to deal with multiple/different input modalities (\ie RGB-D).

\begin{figure*} 
    \centering
  \subfloat{%
       \includegraphics[width=0.47\linewidth]{images/smtl-training-crop.pdf}}
    \hfill
  \subfloat{%
        \includegraphics[width=0.47\linewidth]{images/smtl-test-crop.pdf}}
  \caption{The Sequential Multi-Task learning problem. During training (left) a sequence of tasks are presented to the network, one by one. For each task, a set of task-specific parameters are learned (colored blocks), freezing the shared ones (grey blocks). During inference (right) task-specific parameters are to the network allow to solve multiple tasks on demand with a low overhead in terms of memory requirements. }
  \label{fig:SMTL} 
\end{figure*}
%An interesting approach is designing models that introduce task-specific network parameters \cite{rebuffi_1, rebuffi_2, packnet, piggyback, quantized}. 
%This approach consists in adding few extra task-specific parameters that are optimized during training on that task, while the other network's parameters are kept frozen. Interestingly, these methods obtain performances comparable to fine tuning the whole network on the new tasks without suffering catastrophic forgetting and at the cost of introducing only a small fraction of the network's parameters per task (between 3\% and 15\%).

%Many mainstream approaches for adapting deep models to novel tasks do not respect the constraints of the robotic setting. For example, fine-tuning the network parameters to the new task produces a powerful model on the novel task but it degrades the performances on the old ones. To avoid this problem, one can think to replicate the network and train a separate copy for each new task. This approach preserves exactly the performances on the old tasks at the expense of introducing as many copy of the network's parameters as the number of the tasks to be performed, and this should be avoided, because it does not scale on systems with limited resources as robots are.

%\fabio{unire i due paragrafi, e esplicitare che siamo i primi a proporre questo scenario in robotica cpme conclusione che introduce i contributi}

\myparagraph{Contributions.}
{To summarize, the contributions of this work are three-fold.
\begin{itemize}
    \item We propose the first benchmark for \fabio{REPLACE sequential multi-task learning} in  robotics, the RGB-D Triathlon challenge. 
    %It aims to motivate researchers in developing new models able to perform different visual tasks on the constrained, realistic robotic setting.
    It considers different input modalities and three fundamental tasks: object recognition, %on the Washington RGB-D Object dataset \cite{rod}, 
    pose estimation % on LineMOD dataset \cite{linemod}, 
    and scene classification. %on NYU Depth V2 dataset \cite{nyu}. %These datasets provide RGB-D images and so, we propose three settings for the challenge: the RGB setting, in which can be used only RGB images, the D setting, in which are only available depth images, and RGB-D setting, where both RGB and depth images are provided.
    %We aim to motivate researchers in developing new models able to perform multiple tasks by sharing many parameters among different tasks and being able to learn sequentially new tasks, without accessing the training data of the other tasks and suffering catastrophic forgetting. 
    %We discuss different metrics that bind the results of the three tasks with the number of parameters used to perform them, and provide the overall score of the challenge. As it is shown in the experiments, we found that the optimal metric is the \textit{Locally Linear Score}. It demonstrates to be the fairest metric and we propose it as the metric for the RGB-D triathlon challenge.
    On the considered dataset, we evaluate several state-of-the art \fabio{SMTL} methods: the serial \cite{rebuffi_1} and parallel \cite{rebuffi_2} residual adapter, Piggyback \cite{piggyback} and Binarized Affine Transfom (BAT) \cite{quantized}.
    \item We propose a new metric for the SMTL task which considers both model accuracy and the memory/computational requirements. 
    %\item We evaluate against the challenge promising methods in the multi-task incremental learning context: serial \cite{rebuffi_1} and parallel \cite{rebuffi_2} residual adapter, Piggyback \cite{piggyback}, and Binarized Affine Transfom (BAT) \cite{quantized}. %These methods are compared with two baseline methods: fine-tuning the whole neural network on the new task, and considering the network as a feature extractor by training only the task-specific classifier. Fine-tuning the network parameters is considered the upper bound for the performances of the methods, while the feature extractor is considered the lower bound.
    \item We release a toolbox enabling researchers to develop their own method for SMTL and compare it with baseline methods. Our code %, which is built on PyTorch, 
    can be found at \url{https://github.com/fcdl94/RobotChallenge}.
\end{itemize}
 
}








==> removing-IL/metrics.tex <==
The \challenge, as we have defined it in section \ref{sec:challenge} implies the need for a new evaluation metric, going beyond the mere comparison of standard accuracies. To this extent, in the following we define a metric which takes into account the two properties we require for a \taskabbrv algorithm, namely: i) single-task performances comparable to the task-specific architectures obtained by fine-tuning, as common practise while%ii) sequentially learning more tasks while avoiding forgetting the knowledge on old ones and iii) 
keeping the number of additional parameters per task as low as possible.

In the following we will review the standard and previous evaluation metrics (\ie \cite{rebuffi_1}) highlighting their drawbacks and proposing a new metric, the \linearscore, overcoming them.

%Defining the accuracy on each dataset is not enough, being a multi-task challenge, the accuracies of the three tasks needs to be joined through single metric that take them into account.
%In particular, the metric must consider two factors: the accuracy achieved in each task and the number of additional parameters required. For example, fine-tuning achieves a very good result but at the cost of using a lot of additional parameters, thus, it should be assigned a low score. The metric must assign a high score when the accuracy is good for all tasks and the additional parameters are few.

%In the discussion it will be used this notation:
%\begin{itemize}
%	\item $a_i^m$ is the accuracy of the model $m$ for the task $i$.
%	\item $a_i^e$ is the accuracy of the feature extractor for the task $i$.
%	\item $a_i^f$ is the accuracy of the fine-tuning for the task $i$.
%	\item $p^m_i$ is the size of the additional parameters (in bit) added by the model $m$ to perform task $i$.
%	\item $\rho_0$ is the size of the base parameters of the model (in bit); these parameters are the ones shared between all tasks.
%\end{itemize}

\myparagraph{Average Accuracy}
The most straightforward metric is the average accuracy per-task. Considering the single per-task evaluation metrics to be directly comparable (\ie normalized on the same range and with the same positive direction), we can compute the final performance score $S$ as:
\begin{equation}
    S = \frac{1}{N}\sum_{t=1}^N \alpha_t.
\end{equation}
Obviously, this choice as the drawbacks of not considering i) the difficulty of each task and ii) the number of additional parameters required for each task.

\myparagraph{Decathlon Score}
%As a starting point, we discuss the metric used in the 
In order to consider the difficulties of each task, we can use the Decathlon Score \cite{rebuffi_1}. This metric has been defined for the Visual Decathlon Challenge \cite{rebuffi_1} in order to properly weight how a model performs in all tasks, penalizing models with good performances on just few scenarios. % and we will call it Decathlon score. 
% define the metric they do not consider the accuracy but the error $E_i$. These are obviously bound by the relation $E_i = 100 - a_i$. Given $\Phi_i(x)$ the function of the neural network for the task $i$, $D_i^{test}$ the dataset to be evaluated for the task $i$, the error $E_i$ of the dataset can be computed as follow:
%\begin{gather}
%	E_i = \frac{1}{|D^{test}_i|} \ \sum_{(x,y) \in D^{test}_i} 1(y \neq \Phi_i(x)).
%\end{gather}
The metric is based on the definition of a minimal accuracy per task $\alpha_t^{\text{min}}$ under which the score assigned for the task $t$ is zero. The minimal accuracy is defined as half the performances of the fine-tuned model $\alpha_t^{\text{FT}}$, namely: $a\alpha_t^{\text{min}}=\text{max}(0,2*\alpha_t^{\text{FT}}-100)$, \ie the accuracy obtained by doubling the error obtained by the task-specific fine-tuned architecture. %can be committed for each task $E_i^{max}$. If $E_i$ is bigger than $E_i^{max}$ the score assigned to the task $i$ is zero. 
The overall score is computed as follows:
\begin{gather}
	S = \sum_{t=1}^{N}\eta_t \ \text{max} (0, \alpha_t - \alpha^{\text{min}}_t)^{\gamma_t},\\
	\alpha_t = 1000\cdot( 100 - \alpha^{\text{min}}_i)^{-\gamma_i}
\end{gather}
where $\gamma_t$ is a coefficient set to 2 in \cite{rebuffi_1}. The score the parameter $\eta_t$ normalizes the score of each dataset in order to be in the range $[0,1000]$. 
It encourages getting a good score on all tasks by raising the difference between errors by a coefficient $\gamma_i$. %In the Visual Decathlon Challenge \cite{rebuffi_1} it is suggested to set $\gamma_i = 2$ for all tasks. 
The advantage of this score is that it considers the difficulty of each task. This means that if a model has very good performances on just few tasks it will get a low decathlon score. 

Contrary to the average accuracy, this metric takes into account the complexity of each task. Nonetheless, it does not contain any dependency on the number of additional parameters per-task. A simple inclusion of the parameters would be possible by considering the following revised version of the score:
\begin{equation}
	S = \sum_{t=1}^{N}\eta_t\cdot \lambda^{-\frac{\rho_t}{\rho_0}}\cdot \ \text{max} (0, \alpha_t - \alpha^{\text{min}}_t) ^{\gamma_t}
\end{equation}
where $\lambda>1$ is a hyper-parameter regulating the impact of the number of additional parameters (\ie the higher is $\lambda$, the higher is the impact of the parameters) and $\rho_0=|\theta_0|$ denotes the memory required by the shared parameters. We set $\lambda=10$ in our experiments.

%\subsection{Revised Decathlon Score}
%This new metric is built upon the decathlon score. It considers the number of additional parameters used while keeping the advantages of the previous metric.
%First of all, it takes into account the accuracy and not the error as done before. Thus, it is introduced a parameter $A_i^{min}$ that represents the minimal accuracy that a model must get to have a score higher than zero for task $i$, and a parameter $A_i^{max}$ that represent the accuracy threshold that guarantees the highest score for task $i$.
%Then, it is introduced another parameter: the minimal number of parameters required by the model $\rho_i$ for the task $i$. 

%The parametric function to compute the score is the following:
%\begin{gather}
% S =  \sum_{i=1}^{N}  \alpha_i \cdot \lambda^{\frac{\rho_0}{\rho_i^m} -1} \cdot max (0, a_i - A_i^{min})^{\gamma_i},\\
%\alpha_i = 1000(A_i^{max}-A_i^{min})^{-\gamma_i}
%\end{gather}

%As it can be noted, the function above contains the hyper-parameter $\lambda$ that did not appear in the decathlon score. $\lambda$ affects the impact of the number of additional parameters. If it is big, then the ratio $\frac{P}{\rho_i^m}$ will be very important for the final score. Otherwise, if it is nearly one, the ratio has only a little effect. $\gamma_i$ and $\alpha_i$ have the same meaning as in the decathlon challenge, and as it was done there, $\gamma_i$ is set to 2 for all the tasks.
This metric preserves the positive aspects of the decathlon score but considering also the number of additional parameters required by the model. However it has a lot of hyperparameters to set (e.g.~$\lambda$,$\gamma$,$\alpha$) and it does not take into account the improvement that a model produces with respect to the feature extractor baseline. % both the parameters and the accuracy, motivating the models to achieve good results in all datasets instead of focusing only on some. Anyway, it requires a lot of parameters to be set: $A_i^{min}$, $A_i^{max}$, $\rho_i$, and $\lambda$. We evaluated some different settings and we propose the following values.
%\begin{itemize}
%	\item $A_i^{min} = 100 - 2(100 - a_i^f)$. It is the minimal accuracy that corresponds to an error equals to the double of the fine-tuning error, as described in the previous score but expressed in term of accuracy.
%	\item $A_i^{max} = 100$. As adopted in the decathlon score.
%	\item $\rho_i^{max} = \rho_0$. We decided to set the value to the number of parameters shared by the network between tasks.
%	\item $\lambda = 10$. We decided to strongly penalize the use of additional parameters.
%\end{itemize}

\myparagraph{\linearscore}
In this work we propose an additional metric that considers both the number of parameters and the accuracy and gets rid of the hyper-parameters required by the decathlon-based scores. It is computed through the following formula:
\begin{equation} 
S=\frac{1000}{N}\sum_{t=1}^{N}\text{max}(0,1-\frac{\rho_t}{\rho_0})\cdot\frac{\text{max}(0, \alpha_t-\alpha_t^{\text{FE}})}{a_t^{\text{FT}}-\alpha_t^{\text{FE}}}
\end{equation}
where $\alpha_t^{\text{FE}}$ is the accuracy of the feature extractor model \ie a model where $\theta_t=\empty$ and only the classifier $\omega_t$ is trained. This metric can be defined in two terms, corresponding to the two $\text{max}$ operations. The first element penalizes the addition of task-specific parameters: if the network do not add any parameter, the score obtained from the accuracies will be kept entirely, otherwise it will be rescaled linearly with the number of per-task additional parameters, until the score is zeroed if the added parameters is equal to the shared ones (\ie the network double its size).  
%This metric penalizes the addition of extra parameters, in fact, it decreases the score when the additional parameter size increases. The maximal size of the additional parameters $\rho_i^m$ allowed to get a score is equal to the number of shared parameters $\rho_0$. 
%For example, the fine-tuning, that copies the original network introducing a number of parameters equals to the original network. 

For the accuracy component, the rationale is the same. Since we want the performances to be at least better than the ones obtained by the feature extractor baseline, we set the score to zero if $a^m_i\leq \alpha^e_i$. At the same time, we use the performance distance among the feature extractor and the task-specific architecture $a^f_i$ as a normalization factor to check how well the model is able to fill the gap between the task-agnostic baseline and the task-specific counterpart. 
%The accuracy is bound linearly to the score. When the accuracy reaches $A^{max}_i$, the model gets an optimal score for that task: 1000. the maximal score is kept unbounded, giving a bonus to the methods that perform better than fine-tuning. On the other hand, if the accuracy is less than or equal to $A^{min}_i$, the model will score zero.

%As in the previous metrics, the parameters need to set carefully. We propose to set $ \alpha^{max}_i $ equals to the fine-tuning accuracy to best evaluate the method. This is very important for a lot of methods, such as piggyback, where the initialization of the backbone network is crucial for the performances of the method itself. We want to avoid that a simple tuning of the backbone network weights increases the score, otherwise methods will be not comparable.
%This requires that each submission to the challenge must compute the fine-tuning accuracy of its backbone network. 
%For the same reason, we set the $A^{min}_i$ equals to the feature extractor accuracy.
%The Equation \ref{eq:ps1} thus becomes:
%\begin{gather} 
%S=\frac{1}{N}\sum_{i=1}^{N}2\cdot(\frac{\rho_0}{\rho_0+p^m_i}-\frac{1}{2})\cdot\frac{max(0, \alpha^m_i-a_i^e)}{a^f_i-a_i^e}
%\end{gather}
%where $a_i^e$ is the accuracy of the feature extractor and $a^f_i$ the accuracy of the fine-tuning for the i-th task. 

As a good practice, since different hyperparameters may lead to different performances of the feature extractor and the fine-tuned architecture, we strongly encourage authors to get the values of $\alpha^{\text{FE}}_t$ and $\alpha^{\text{FT}}_t$ from their own experiments: this will ensure a fair computation of the score and, consequently a fairer comparison with other algorithms.

Finally, we highlight that while in the current version of the challenge $N=3$, the evaluation metrics we have defined generalize to any number of tasks, allowing easy extensions of the challenge. %Moreover, we \textit{do not} specify any fixed order for the tasks: this choice allows researchers to experiment with different sequences, with the possibility of exploring the relation among the tasks.


\begin{table}[t]
\centering
\caption{A comparison of the properties of \taskabbrv metrics}% taking into account different factors}
\label{tab:metrics}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|cccc}
\multicolumn{1}{l|}{} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}considers \\complexity\\of tasks\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}penalizes\\addition\\of parameters\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}compares\\to feature\\extractor\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}compares\\to fine\\tuning\end{tabular}} \\ \hline
ave. accuracy & \xmark & \xmark & \xmark & \xmark \\ \hline
decathlon & \cmark & \xmark & \xmark & \cmark \\ \hline
rev. decathlon & \cmark & \cmark & \xmark & \cmark \\ \hline
linear & \cmark & \cmark & \cmark & \cmark \\ \hline
\end{tabular}}
\end{table}

==> removing-IL/related.tex <==
Our work is related to many previous studies in the area of visual learning, e.g. those addressing the problems of transfer and multi-task learning. Moreover, since we process multiple modalities (RGB and depth images), our work is also linked to multimodal learning. In the following we first review recent benchmarks
proposed in computer and robot vision and involving multiple tasks. Then, we describe the relation between our work and previous studies on transfer, multi-task and multimodal learning. In the following we consider only deep neural models, due to their clear advantages in terms of performance with respect to shallow models.

\myparagraph{Learning from Multiple Tasks/Domains: Benchmarks.}
%Visual Challenges. 
%STANDARD CHALLENGES
Benchmarks are fundamental tools to advance research in visual recognition and robot perception. %fundamental components of a research community. 
%Models addressing challenges such as 
For instance, in robot vision, datasets as SeqSLAM \cite{milford2012seqslam}, RGB-D SLAM \cite{sturm2012benchmark}, allowed the development of methods for addressing loop-closing, SLAM \cite{mur2015orb} and semantic mapping \cite{sunderhauf2017meaningful}.
%dobbiamo mettere lavori e datasets che fanno tasks come Visual SLAM e loop closing
%
In computer vision, datasets and challenges as ImageNet \cite{imagenet}, Common Objects in Context (COCO) \cite{lin2014microsoft} and Places \cite{zhou2018places} have brought significant progresses, enabling to learn deep architectures which are not only effective for a single categorization problem % have been built for 
but they can also serve as general purpose models to address other recognition tasks % to the entire community
\cite{krizhevsky2012imagenet}. %Usually, these benchmarks focus on a single task, evaluating each model with the task specific performance metric (\eg accuracy for classification or mean average precision for detection). 

Recently, the idea of learning universal representations \cite{bilen2017universal} and task-agnostic deep models, \ie neural architectures which should perform well over multiple tasks and/or domains, %at the same time, % need for robust visual model 
has attracted the attention of several researchers \cite{rebuffi_1,quantized} fostering the creation of new datasets and challenges. 
%to propose challenges where a single model should perform well over multiple domains at the same time. 
A notable example is the Robust Vision Challenge\footnote{http://www.robustvision.net}, which aims to facilitate the development of robust models, \ie models which must perform well on a specific problem (\eg depth estimation, semantic segmentation) but on different settings (\eg environments, sensors). % evaluated on multiple datasets at the same time. 
Another interesting benchmark is the Visual Domain Decathlon \cite{rebuffi_1}, which promotes %the goal is to produce 
the developments of SMTL models considering ten different categorization problems. Drawing inspiration from these initiatives in the computer vision community, in this paper we propose a novel benchmark to stimulate research in robot perception. In particular, we respect to the aforementioned SMTL benchmarks, we consider a setting where i) the task to be addressed are different (namely, pose estimation, object recognition and scene classification); ii) the evaluation protocol is newly designed, in order to take into account not only the per-task performances but also
the computational complexity of the model; %the number of additional parameters needed by a model; 
iii) different input modalities are considered (\ie RGB, Depth and RGB-D).

\myparagraph{\taskName. } Given a pretrained model and a set of tasks whose data are available in \textit{different} times, the goal of \taskName \cite{piggyback,quantized} is to learn a network able to address all tasks while keeping low the overhead in terms of required parameters. In computer vision, this task has been tackled by methods addressing the aforementioned Visual Domain Decathlon challenge~\cite{rebuffi_1,rebuffi_2,piggyback,quantized}. These models differ on how they extend a pretrained model to new tasks, considering for instance adding task-specific network modules~\cite{rebuffi_1,rebuffi_2} or changing the network parameters by means of binary masks \cite{piggyback,quantized}. In robot perception, this task has not been addressed yet, thus we will take these models as baseline approaches.

\myparagraph{Multi-Task and Transfer Learning. }
%\fabio{unire prossimi 3 paragrafi}
The formulation of our task is strictly related to other problems such as MTL and transfer learning. Similar to ours, the goal of MTL is to train a model on multiple tasks. %together, with the aim of both having a single model able to tackle all the tasks at the same time and to exploit the relationships among the tasks to improve the per-task performances \cite{Caruana1997}. %The possibility of producing a model able to solve multiple tasks at the same time, is particularly attractive for robotics where saving computational resources is crucial. For these reasons, 
Different works addressed MTL in various contexts of robot perception, ranging from reinforcement learning \cite{devin2017learning}, learning from demonstrations \cite{rahmatizadeh2018vision}, grasping \cite{fang2018multi} and scene understanding \cite{teichmann2018multinet}. Differently from the MTL setting, we focus on the sequential setting, \massi{where we do not have access to the data of all the tasks beforehand but we receive them one after the other, sequentially}. %multiple tasks are learned but one after the other \cite{packnet,quantized} and focusing are attention also to the number of additional parameters per-task used.

%\myparagraph{Incremental Learning. } 
\massi{REPLACE WITH TL SMTL is also closely related to incremental learning \cite{thrun1998lifelong}. Similarly to incremental learning our aim is to progressively add knowledge to a model without forgetting the previously learned concepts, overcoming the problem of catastrophic forgetting~\cite{french1999catastrophic}. Differently from the incremental and the incremental class learning problems \cite{lomonaco2017core50,valipour2017incremental,camoriano2017incremental,turkoglu2018incremental} we want to add tasks to the network and not consider new categories, thus we need a separate output space for each new task.}% For this reason, in SMTL also the catastrophic forgetting problem is tackled by training only task specific parameters, added for each new task~\cite{rebuffi_1,rebuffi_2,piggyback,quantized}. %However, researchers may exploit the relation among tasks while training their models (\eg \cite{rusu2016progressive}): we did not impose any fixed order for learning the tasks.
%This problem is relevant in robotics as shown by recent efforts on proposing datasets \cite{lomonaco2017core50} and algorithms \cite{valipour2017incremental,turkoglu2018incremental}, we tackle a different proin SMTL the models usually consider training only task specific parameters, for each new task. thus i) Our challenge considers learning sequentially multiple tasks, thus a model needs to tackle the catastrophic forgetting problem. In the sequential multi-task learning literature this is usually achieved by considering task-specific components, with the components of each task learned independently~\cite{rebuffi_1,rebuffi_2,piggyback,quantized}. However, researchers may exploit the relation among tasks while training their models: we did not impose any fixed order for learning the tasks.% on our setting, thus it is possible to start by first learning tasks which are beneficial to others.

%\myparagraph{Multi-Task Learning. }
%The focus of our task strictly relates to multi-task learning (MTL) \cite{Caruana1997}. In MTL, the  goal is to train a model on multiple tasks together, with the aim of both having a model able to tackle all the tasks at the same time and to exploit the relationships among the tasks to improve the per-task performances \cite{Caruana1997}. The possibility of producing a model able to solve multiple tasks at the same time, is particularly attractive for robotics where saving computational resources is crucial. For these reasons, different works addressed this task in robotics and in various contexts such as reinforcement learning \cite{devin2017learning,hamaya2017learning} and robot vision \cite{fang2018multi,rahmatizadeh2018vision}. Differently from the standard definition, we focus on the sequential setting, were multiple tasks are learned but one after the other \cite{packnet,quantized} and focusing are attention also to the number of additional parameters per-task used.

%\myparagraph{Transfer Learning. } ????
% 

%\myparagraph{\massi{Multi-modal learning.} }
%The possibilities of using RGB and/or depth information, naturally involves understanding how to merge these two modalities. Recent years multiple efforts have been devoted on understanding how to elaborate depth information with a network pre-trained on RGB images \cite{eitel2015multimodal}. These approaches are based on different strategies, involving either pre-processing depth images \cite{bo2013unsupervised,aakerberg2017depth} or learning based approaches \cite{eitel2015multimodal,gupta2016cross,carlucci2018deco}. To this extent, our proposed challenge will allow studying the effectiveness that multimodal fusion approaches has over multiple tasks and in which extent the fusion strategy learned for a task can help/may benefit from the transformations learned on the others.

%\massi{IMPORTANCE OF BENCHMARKS}
%In recent years, the computer vision community has proposed challenges and competitions such as ImageNet Large Scale Visual Recognition Challenge (ILSVRC) \cite{imagenet}, Common objects in context (COCO) \cite{lin2014microsoft}, Places \cite{zhou2018places}. These competitions have encouraged the researchers in developing new methods that led to improvements in object recognition, object detection, semantic segmentation, place recognition, and visual question answering. The challenges motivated the researchers with interesting problems, provided new datasets and evaluation metrics to establish which method solved best the problem.

%\massi{MULTI-DOMAIN/MULTI-TASK BENCHMARKS}
% The robotics community has seen a great opportunity in the growth of the computer vision and especially of the deep learning methods. In the last few years, researchers were very engaged in discussing how deep learning could be applied and what are the opportunities that it offers in the robotic field \cite{brock2018issuesRV}. 
% For instance, \cite{levine2018learning, schwarz2018rgb} demonstrate the use of deep learning for grasping and manipulating objects. \cite{levine2018learning} describes an approach that learns eye-hand coordination for robotic grasping using a monocular camera and a convolutional neural network that predicts the probability of success of the grip. \cite{schwarz2018rgb} presents a deep learning approach that combines object detection and semantic segmentation to perform autonomous robotic manipulation in cluttered scenes. 
% Moreover, 10\% of the papers submitted to ICRA 2018 used as keyword \textit{Deep learning in robotics and automation}, and it was initiated a new Conference on Robot Learning (CoRL).

%\massi{BENCHMARKS on ROBOT VISION}
%However, even if robotic context can take advantage of the progress in computer vision, it presents a different scenario. Differently, from computer vision, where the agent is static and has the goal to extract information over images, a robot is a dynamic agent that acts in, and interacts with, the world with the goal to make decisions and perform actions. It introduces many more challenges such as the deployment in open-set conditions, incremental learning, semantic reasoning, active learning, active vision, and transfer learning. 

%Researchers still lack benchmarks to evaluate the performance of the deep learning methods they develop in this new context. This theme is very important for the robotics community, in fact, it was discussed recently in the main conferences. In CVPR 2018 it was held a workshop named \textit{Real-World Challenges and New Benchmarks for Deep Learning in Robotic Vision}\footnote{https://sites.google.com/view/cvpr2018-robotic-vision/home} in which were discussed new benchmarks with the aim of recreating the success of the computer vision challenges also in robotic vision.
%In this work we aim to contribute to the development of new method in the robotic scenario by proposing a new evaluation protocol for deep neural networks in the context of multi-task incremental learning.

%\massi{MULTI-MODAL}

%\massi{MULTI-TASK/MULTI-DOMAIN WORKS}
%\massi{DESIRABLE PROPERTIES}

%Multi-task learning has been proven to be effective in deep learning by Caruana \cite{Caruana1997}. This work proposes a neural network that shares weights in the early layers and defines specialized ones in the later layers. The network parameters are jointly learned by interleaving samples from each task. It demonstrates that sharing parameters is useful because tends to regularize better the network, improving generalization and performances. However, this approach has many limitations: it requires many additional parameters per task, it requires to manually design the network deciding which layers should be shared across tasks, and adding a novel task when the model has been already optimized requires to train again the whole network from scratch by accessing the old training data.

%An important research area in multi-task learning deals with networks able to learn sequentially new tasks. Works in this area present approaches in which are developed deep neural networks able to learn incrementally \cite{rebuffi2017icarl, aljundi2017memory}. It is crucial, while learning a new task or domain, to keep the same performances on the already learned tasks. Ideally, every time a new task has to be learned, it should share the parameters with the old tasks, adding as few task-specific parameters as possible, without suffering \textit{catastrophic forgetting} \cite{catforg_1, catforg_2} and without accessing the old training data.


%We can identify two strategies to avoid catastrophic forgetting: one is to preserve the knowledge of the old tasks without adding extra parameters, the other is to freeze the weights of the old tasks while learning additional task-specific parameters.
%Methods that follow the first strategy are for example \cite{li2017learning} and \cite{ewc}. In \cite{li2017learning}, the authors ensure the preservation of performances on previous tasks by using initial network responses on new data as regularization targets during the new task training. \cite{ewc} considers updating the network parameters based on the importance for previously seen tasks.
%While these methods do not increase the network size maintaining the same number of parameters as the original network, performance drops as many tasks are added to the network, limiting the number of learned tasks and suffering catastrophic forgetting. Also, for \cite{li2017learning}, a large domain shift for a new task causes a significant drop in prior task performance.
%To overcome these issues, methods that follow the second strategy keep the previous weights frozen while adding additional per task parameters, leaving untouched the performances on previous tasks and avoiding catastrophic forgetting. The extreme interpretation of this strategy can be found in \cite{rusu2016progressive}. It instantiates a parallel neural network for each new task, connected to networks of other tasks through parallel connections. The main drawback of this method is clearly the significant growth of parameters for every task added.
%However, recently were introduced methods that follow the second approach capable of learning a new task by introducing only few task-specific parameters. These methods were first proposed in the context of \textit{multiple domain learning} (MDL). The main goal of that setting is to learn a single network that can represent compactly many the domains introducing a minimal number of task-specific parameters. Bilen and Vedaldi \cite{BilenV17} proposed to share all core network parameters except normalization layers to model different domains in a single neural network, \cite{packnet} introduced an approach that uses weight-based pruning to free up redundant parameters across all layers of deep neural network with minimal loss in accuracy, \cite{dan} proposed a parameter efficient architecture that enables learning new domains sequentially without forgetting. 
%Recently, a new challenge, named the Visual Decathlon Challenge \cite{rebuffi_1}, was introduced, motivating researchers to develop new powerful methods: Piggyback \cite{piggyback}, binarized affine transformation (BAT) \cite{quantized}, series \cite{rebuffi_1} and parallel \cite{rebuffi_2} residual adapters.
% espandere questi metodi?

%In this work we investigate these methods and we assess their performance against our challenge, proving that they can achieve good performances also in the multi-task incremental learning scenario. 

==> removing-IL/results.tex <==
\label{sec:experiments}

In this section we test state-of-the-art \taskabbrv algorithms \cite{rebuffi_1,rebuffi_2,piggyback,quantized} on our \challenge. In the following we present the baseline methods,  provide the implementation details and we discuss the obtained results. 

\subsection{Baselines}
\label{sec:baselines}
We consider six methods: \textit{fine-tuning}, \textit{feature extraction}, \textit{series} \cite{rebuffi_1} and \textit{parallel residual adapters} \cite{rebuffi_2}, \textit{Piggyback} \cite{piggyback}, and \textit{binarized affine transformation (BAT)} \cite{quantized}. The first two are the simplest transfer learning strategies, while the others are the state-of-the art models for \taskabbrv.

\textit{Fine-tuning} (FT) %is the simplest method for transfer learning. It 
requires to copy the full architecture and training it on the new task of interest. %It requires to instantiate a new ResNet-18 model pre-trained on the ImageNet dataset for each task and each of them is fed with the images of the respective dataset. 
Since this procedure is repeated for each task, this method produces %is trained independent of the others, both in training and evaluation phases, de-facto producing 
three different models, one per-task.

\textit{Feature extraction} (FE) keeps a single backbone architecture but, for each tasks instantiates a new output layer.  %that requires only one backbone neural network but three different classification layers. 
The weights of the network are frozen, i.e. they are not optimized, besides the task-specific output layer.

For what concerns the \taskabbrv models, in the \textit{series residual adapter} (RS)~\cite{rebuffi_1} a residual adapter module is added in series after the convolutional layer of each residual unit.  %While the weights of the backbone networks are taken from the pre-trained model on ImageNet dataset, the series adapter modules' convolutional layers are initialized randomly and follow the normal distribution $\mathcal{N} (0, 0.0001)$ and the batch normalization layers are initialized to have scale equals 1 and bias equals zero. Each task requires a few additional parameters that are learned independently from the other tasks with stochastic gradient descent with momentum. All the batch normalization layers are considered task-specific.
Similarly, in \textit{parallel residual adapter} (RP)~\cite{rebuffi_2} the task-specific modules are added in parallel to the convolutional layers of each residual blocks and not serially. In both cases, the residual adapter is implemented as a convolutional layer with kernel size $1 \times 1$ (plus a batch normalization layer in \cite{rebuffi_1}). %Instead of adding the residual adapter modules in series, it adds task-specific residual adapter modules parallel to the convolutional layers of each residual blocks. Each parallel residual adapter module consists in a small convolutional filter with kernel size $1 \times 1$.%Instead of adding serial residual adapter modules, it adds task-specific residual adapter modules parallel to the convolutional layers of each residual blocks. Each parallel residual adapter module consists in a small convolutional filter with kernel size $1 \times 1$. %%whose parameters are initialized randomly and follows the distribution $\mathcal{N} (0, 0.0001)$. The other parameters are taken from the pre-trained model. Also for this method, the batch normalization layers are considered task-specific.

\textit{Piggyback} (PB)~\cite{piggyback} make use of task-specific binary masks that are added to each convolutional layer of a backbone network. These binary masks multiply point-wise the original network weights, de facto producing new convolutional filter for the task of interest. %The real-valued masks parameters are initialized to $0.01$ and the threshold value is zero. The other parameters are taken from the pre-trained model and the batch normalization layers are considered task-specific.

\textit{BAT}~\cite{quantized}, similarly to \cite{piggyback} uses task-specific binary masks that are paired with each convolutional layer of a backbone network. Differently from~\cite{piggyback} the masks are not applied through a point-wise multiplication but are used to perform an affine transformation of the convolutional filters, creating a new set of task-specific weights. 
%The real-valued masks parameters are initialized randomly and follow a uniform distribution $\mathcal{U}(0.00001, 0.00002)$. The parameters $k_1, k_2, k_3$ are task-specific and are optimized while training for the specific task. They are all initialized to zero. The parameter $k_0$ is set to 1 and it is not learnable.

\subsection{Implementation}
%Each model starts from the same network: a ResNet-18 \cite{resnet} model pretrained on ImageNet.
All the methods we evaluate start from a pre-trained architecture. We decided to use the \textit{ResNet-18}~\cite{resnet} pre-trained on ImageNet~\cite{imagenet}. This network has been chosen as a trade-off between accuracy and speed.
%The various methods evaluated against the challenge in this work require a backbone network. We decided to use the \textit{ResNet-18}~\cite{resnet} pre-trained on ImageNet \cite{imagenet} dataset as a starting point for each method. This network has been chosen as a trade-off between accuracy and speed. %Moreover, being a very common choice, it is available in many deep learning frameworks, which is important for ensuring a fair and straight-forward comparison with our baselines.%many frameworks provide their own implementation and even some pre-trained models, and this can help other researchers to replicate the results reported in this work or to build over them.

%todo come viene trattato il caso RGB-D (da aggiornare con Surface e FusionNet (possiamo citare il lavoro) )
% inserire come trattiamo la depth (ovvero la coloriamo con surface++ e usiamo Fusion Net) come detto sopra, dove si parla dei RW di ROD)
All the methods have been evaluated on three input modalities: RGB only, depth only and using both RGB and depth.
To handle the depth images we took inspiration from \cite{aakerberg2017depth}, coloring the depth images using their proposed method, called Surface++. For the single modality case, we take as backbone network architecture a ResNet-18 previously described. % \cite{resnet} pre-trained on ImageNet, 
For the RGB-D setting we fuse (by concatenation) the features of two ResNet-18, one processing only RGB images and the other only depth maps. %pre-trained on ImageNet and 
The fused features are passed through a fully connected layer that we use as the output layer, similarly to \cite{eitel2015multimodal}. %To fuse the features we just concatenate them.

%hyper-parameters
To provide comparable results among the baselines, the same set of hyper-parameters is used for all the methods in each task. The networks are trained using Stochastic Gradient Descent with momentum (SGD) except for Piggyback and BAT where SGD is used for the classification layer and Adam \cite{kingma2014adam} is used for the rest of the network, as suggested by their authors \cite{piggyback, quantized}.
The various methods are trained for 30 epochs in each setting, with a batch-size of 32, weight decay of $5\cdot10^{-5}$. %0.00005. The learning rate of the SGD optimizer is set to 0.005 for every task and method, while we have to adapt the Adam learning rate for every task, using 0.00001 for ROD, 0.00005 for LineMOD and 0.00010 for NYU. The learning rates are decayed by a factor of 10 after 20 epochs. 
The learning rate of the SGD optimizer is set to 0.005 for every task and method, while we have to adapt the Adam learning rate for every task, using $1\cdot10^{-5}$ for ROD, $5\cdot10^{-5}$ for LineMOD and $1\cdot10^{-4}$ for NYU. The learning rates are decayed by a factor of 10 after 20 epochs. 

% data preprocessing per i tre dataset 
% The three datasets offer RGB-D images of different sizes: the RGB-D object dataset contains images of size nearly $100 \times 100$ pixels, LineMOD cropped dataset contains images of size $64 \times 64$ pixels, and NYU Depth V2 Dataset contains images of size $640 \times 480$ pixels. To make use of them with the neural network it is necessary to rescale the images all to the same size: $224 \times 224$ pixels, that is the minimal dimension accepted by the implemented ResNet. The data were normalized  by subtracting the mean of the ImageNet dataset to each channel. To increase the generality of the dataset, data augmentation was performed: the images of RGB-D object dataset are cropped randomly, while images of NYU Depth V2 Dataset are cropped randomly and mirrored (i.e. flipped horizontally).

To implement all the baselines we used the \href{pytorch.org}{PyTorch} framework. %that offers an open-source implementation of the ResNet-18 and a pre-trained model on the ImageNet dataset. 
The code of the networks and the training procedure can be found here: \url{https://github.com/fcdl94/RobotChallenge}.

\subsection{Results}

%%%%% Comparison with the state of the art %%%%%%%
\myparagraph{State of the Art for each tasks}
In order to better understand the results of our baselines, in table \ref{tab:sota} we report a comparison on the RGB-D setting between the state of the art methods for each task and a fine-tuned ResNet-18.% we used as backbone network, fine tuned on the specific dataset.
%%% ROD %%%
%In the last years many works were developed to solve this task. We will focus on deep convolutional neural networks (CNN) methods that can be applied to the different settings we propose, in particular to the RGB-D. One of the first methods that applied CNNs in RGB-D object recognition was \cite{socher2012convolutional} that uses a combination of CNNs for feature extraction and Recursive Neural Networks (RNNs) for classification. Then, there were proposed many methods to color depth images \cite{eitel2015multimodal, wang2016correlated, aakerberg2017depth, carlucci2018deco}. Eitel et al. \cite{eitel2015multimodal} proposed a multi-modal network based on two pre-trained CNNs that were fine tuned to the RGB-D Object Dataset \cite{rod}. To make use of the parameters learned in the RGB mode and applied to depth images, the authors evaluated different encoding methods of the depth images among which Jet color encoding showed the best performance. \cite{wang2016correlated} jointly learns feature representations from raw RGB-D data with a pair of deep neural networks to better exploit sharable and modal-specific information. Moreover, they proposed to color the depth data by computing the surface normal for each pixel. \cite{aakerberg2017depth} proposes an improvement of FusionNet \cite{eitel2015multimodal} by coloring the depth images by computing the surface normal and using a deeper network architecture.  \cite{asif2018multi} proposes a novel framework to learn a discriminative and spatially invariant classification model for object and indoor scene recognition.

For ROD \cite{rod} we report the top three methods \cite{li2015hybrid, carlucci2018deco, aakerberg2017improving}. \cite{aakerberg2017improving} uses an ensemble of deep models, extracting depth information through different colorization techniques. \cite{carlucci2018deco} proposes a deep architectures that learns how to map depth data to three channel images. \cite{li2015hybrid} extract depth data and encode it as Fisher vectors, without using colorization. %%% LINEMOD %%%
% In the literature there are many works that address this task, from \cite{schneiderman2000statistical, pepik2012teaching, hejrati2014analysis} to more recent methods that use Convolutional Neural Networks (CNN) \cite{wu2016single, pavlakos20176, su2015render, tulsiani2015viewpoints, learningdescriptors, poseregression}. The CNN-based methods use very different approaches. For instance, there are methods that treat pose estimation as a classification problem, fragmenting the pose space into bins. These methods can be divided into two groups: the first contains those that predict 2D keypoints from the image and then use a 3D model to evaluate the 3D pose given these keypoints \cite{wu2016single, pavlakos20176}; the second group contains those methods that predict directly the pose given the image \cite{su2015render, tulsiani2015viewpoints}.
%An interesting method is the one in \cite{learningdescriptors}. It uses a CNN to map the image space to a descriptor space and then searches, through the nearest neighbor algorithm, the most similar descriptors to predict the pose and the object class.
%There exist also CNN-based methods that consider pose estimation as a regression problem. The challenge is that 3D pose space is a non-Euclidean space, hence, CNN algorithms need to take it into account. To this extent, in \cite{poseregression} the authors try to solve the problem by designing a suitable representation and a loss function that respects the non-linear structure of the pose space. They specifically study two representations of the rotation, axis-angle and quaternions, and model their constraints using non-linearity in the output layer. Moreover, they propose to (i) use the geodesic distance on the space of rotation matrices as a loss function; (ii) exploit the knowledge about the object, proposing a network architecture that is made by part shared between all objects (called feature network) and a part that is object-specific called pose network.
%Taking inspiration from \cite{poseregression}, in this work we represent the rotation using the unit quaternion representation.

For the LineMOD dataset \cite{linemod} we report two state of the art approaches \cite{zakharov20173d, learningdescriptors}. \cite{learningdescriptors} uses a CNN to map the image space to a descriptor space where the pose and object classes are predicted through a nearest neighbour classifier. %and then searches, through the nearest neighbor algorithm, the most similar descriptors to predict the pose and the object class. 
\cite{zakharov20173d} builds upon the previous model, introducing a triplet loss function with a dynamic margin. These works are not directly comparable to ours since they employ slightly different settings (\eg they use also synthetic images), but we report as accuracy measure a metric that consider correct a test sample only if the angular error is below 20 degree.
%%% NYU %%%
%% Despite many works exploit RGB data only to solve this task, we want to focus on methods that analyze both RGB and depth images. The main issue of the RGB-D setting is the lack of annotated datasets that make difficult to train CNNs avoiding overfitting. In the literature can be found two different approaches: adapting pre-trainined RGB CNN models to the depth images by fine-tuning, or focusing on improving the representation of the depth without relying on RGB knowledge. Following the first approach, \cite{zhu2016discriminative} proposes a multi-modal fusion network that consider inter- and intra-modality correlation, \cite{wang2016modality} extracts CNN features using RGB data and two different color encoding of depth data (HHA \cite{gupta2014learning} and surface normals) by fine-tuning pre-trained RGB CNN that are combined with proposal-based Fisher Vector, \cite{gupta2016cross} proposes to transfer supervision between RGB and depth modalities.
%\cite{song2017combining} propose a framework that combines the two approaches, by exploting knowledge acquired from large RGB dataset and depth-specific knowledge learned from the depth images.
%An important work that follows the second approach is \cite{song2017depth} that considers biased the depth features fine-tuned from RGB datasets and proposes to learn from scratch the depth features with the help of depth patches. Finally, an interesting work is \cite{du2018depth} that proposes a two-step training strategy that builds a Res-U architecture on a Generative Adversarial Network (GAN) that translates RGB images to depth ones.

For the NYU Depth V2 dataset \cite{nyu} we report three state of the art methods \cite{du2018depth, song2017combining, song2017depth}. \cite{du2018depth} proposes a two-step training strategy %that exploits a Res-U architecture on a Generative Adversarial Network \cite{goodfellow2014generative} 
that translates RGB images to depth ones. \cite{song2017depth} %considers biased the depth features fine-tuned from RGB datasets and 
proposes to learn from scratch the depth features with the help of depth patches. %\cite{song2017combining} proposes a framework that combines two approaches: adapting pre-trainined RGB CNN models to the depth images by fine-tuning and focusing on improving the representation of the depth without relying on RGB knowledge.

It can be noted that the fine-tuned ResNet-18 is a competitive baseline by itself on each task, confirming the soundness of our choice.


\begin{table}[t]
\caption{
Comparison between ResNet-18 \cite{resnet} fine tuned on the task and state of the art methods in the RGB-D setting.}
\label{tab:sota}
\centering
\resizebox{1.\linewidth}{!}{%
\begin{tabular}{ccccc}
\multicolumn{1}{l}{}                                                    & \multicolumn{1}{l}{}          & \textbf{ROD} & \textbf{Linemod} & \textbf{NYU} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ROD\end{tabular}}            & \multicolumn{1}{c|}{CNN+Fisher \cite{li2015hybrid}}                     &     93.8     & -                & -            \\  
                                                                        & \multicolumn{1}{c|}{(DE)$^2$CO \cite{carlucci2018deco}}                 &     93.6     & -                & -            \\ 
                                                                        & \multicolumn{1}{c|}{FusionNet enhanced \cite{aakerberg2017improving}}   &     93.5     & -                & -            \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Linemod\end{tabular}} & \multicolumn{1}{c|}{Zakharov et al. \cite{zakharov20173d}}            & -            &     93.2 \footnotemark        & -            \\  
                                                                        & \multicolumn{1}{c|}{Wohlhart et al. \cite{learningdescriptors}}   & -   &   96.2  \footnotemark[\value{footnote}]    & -     \\ \hline 
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}NYU\end{tabular}}    & \multicolumn{1}{c|}{Du et al. \cite{du2018depth}}                               & -            & -                &      67.5    \\  
                                                                        & \multicolumn{1}{c|}{Song et al. \cite{song2017depth}}                   & -            & -                &      66.7    \\
                                                                        %& %\multicolumn{1}{c|}{Song et al. \cite{song2017combining}}               & -            & -                &      65.8   \\
                                                                        \hline
Ours                                                                    & \multicolumn{1}{c|}{Resnet-18}                                          &     93.9     &       96.9       &      68.4   \\ \hline
\end{tabular}%
}
\end{table}
\footnotetext{The metric for Linemod keeps into account only the estimation of the rotation}

\myparagraph{Performances on the \challenge.}
{In this subsection, we report the results of all the baselines on our \challenge.
Table \ref{tab:score} reports the scores for each method, setting and metric.
In the table, the \textit{Par.} column reports the ration between the number of task-specific parameters introduced to solve each task and the parameters of the backbone network. We report a single value because all the network architecture introduce the same number of parameters for every task.
%demonstrating that the method with better performance is BAT. Series residual adapter method is comparable with BAT in the RGB-D setting, where it achieves a locally linear score higher of 1 point.
We will discuss the different metrics by focusing on the comparison between BAT and series residual adapters (RS) methods in the RGB-D setting, which are the best performing methods for the residual adapters and mask-based approaches respectively.

Considering the average accuracy metric (AvgA), RS outperforms BAT by far. However, from table \ref{tab:accuracy}, we can see that RS is not the clear winner: even if it achieves a very high accuracy in NYU, BAT outperforms it in LineMOD dataset and they are comparable in ROD. This result underlines that the average accuracy metric does not considers the complexity of the task, encouraging the methods to get very high score in only few tasks.
The two methods get closer in the Decathlon metric (DS) because it considers the complexity of the task and it encourages methods to get good score on all tasks. However, the DS does not penalize the addition of parameters, and by considering them, we note a remarkable change in the scores.
The Revised Decathlon score (RevDS) strongly penalizes the addition of parameters, explaining why BAT exceeds by far RS. Moreover, we can see that RS obtain a score even worse than the other methods, that in the other metrics it outperforms.
Finally, in the locally linear score (LL) the two methods are comparable, underlying the different trade-off between performance and addition of parameters that each method adopt. 
% perche' LL e' meglio di altre a stimare diff. tasks?
It is worth noting that, neglecting the number of parameters, RS would have a greater score. In fact, the locally linear score considers more valuable an increase of the performance where there is a smaller gap between FT and FE (such as in the NYU dataset, where RS outperform BAT) than where there is a larger gap (such as in the LineMOD dataset, where BAT outperform RS). In other words, the methods are comparable in LineMOD because both are able to strongly adapt to the dataset, achieving a result better than the FE by far and obtaining performance similar to the FT.

{Looking at the results for different modalities, the results are pretty confirmed in the Depth and RGB only settings where BAT still outperforms RS. In particular, in the RGB setting, BAT is able to exceed also the fine-tuning baseline, obtaining an outstanding result. We ascribe this behavior to the regularization introduced by training binary masks. %The LL score underline this result by assigning a score that exceed 1000, that is the value obtained by fine-tuning neglecting the additional parameters.
In the Depth setting, RS obtains an excellent result in the NYU dataset, but it performs poorly in the LineMOD dataset, thus, its overall performance is worse than BAT that achieves good results in all the datasets, as it is shown by the LL scores.
}

For completeness, we report in table \ref{tab:accuracy} the accuracy for each method, setting and task.
}

%%%%%%% SotA table %%%%%% 



\begin{table}[t]
\caption{Baselines score for the RGB-D Triathlon challenge. The best method is bold, the second best is underlined.}
\label{tab:score}
\centering
\resizebox{1.\linewidth}{!}{%
\begin{tabular}{ll|c|ccc|c}
\textbf{Setting}                & \textbf{Method}                   & \textbf{Par} & \textbf{AvgA} & \textbf{DS} & \textbf{RevDS} & \textbf{LL} \\ \hline
\multirow{6}{*}{\textbf{RGB}}   & FT                                & 1.00         & {\ul 85.0}    & \textbf{750}  & 8             & 0               \\ 
                                & FE                                & 0.00         & 53.1          & 229           & 229           & 0               \\ 
                                & PB \cite{piggyback}               & 0.03         & 84.6          & 577           & {\ul 463}     & 853             \\ 
                                & BAT \cite{quantized}              & 0.03         & \textbf{85.3} & {\ul 693}     & \textbf{556}  & \textbf{1196}   \\ 
                                & RS  \cite{rebuffi_1}              & 0.16         & 82.6          & 500           & 169           & 818             \\ 
                                & RP \cite{rebuffi_2}               & 0.13         & 83.2          & 542           & 228           & {\ul 922}       \\ \hline
\multirow{6}{*}{\textbf{D}}     & FT                                & 1.00         & \textbf{76.5} & \textbf{750}  & 8             & 0               \\
                                & FE                                & 0.00         & 43.0          & 213           & 213           & 0               \\
                                & PB \cite{piggyback}               & 0.03         & 74.4          & 598           & {\ul 480}     & {\ul 909}       \\
                                & BAT \cite{quantized}              & 0.03         & {\ul 76.0}    & {\ul 741}     & \textbf{595}  & \textbf{957}    \\
                                & RS  \cite{rebuffi_1}              & 0.16         & 74.8          & 582           & 197           & 865             \\
                                & RP \cite{rebuffi_2}               & 0.13         & 72.6          & 501           & 211           & 824             \\ \hline
\multirow{6}{*}{\textbf{RGB-D}} & FT                                & 1.00         & \textbf{86.4} & \textbf{750}  & 8             & 0               \\
                                & FE                                & 0.00         & 55.5          & 237           & 237           & 0               \\
                                & PB \cite{piggyback}               & 0.03         & 84.2          & 451           & {\ul 362}     & 560             \\
                                & BAT \cite{quantized}              & 0.03         & 85.6          & 514           & \textbf{413}  & {\ul 890}       \\
                                & RS  \cite{rebuffi_1}              & 0.16         & {\ul 86.1}    & {\ul 524}     & 177           & \textbf{891}    \\
                                & RP \cite{rebuffi_2}               & 0.13         & 84.5          & 481           & 203           & 818             \\ \hline
\end{tabular}%
}
\end{table}


\begin{table}[t]
\caption{Results in term of accuracy for each task in the RGB-D triathlon challenge. The best method is bold.}
\label{tab:accuracy}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cl|ccc}
\textbf{Setting}                  & \textbf{Method}                                 & \textbf{RGB}          & \textbf{D}          & \textbf{RGB+D} \\ \hline
\multirow{6}{*}{\textbf{ROD}}     & FT                                              & 90.8                  & 83.3                & \textbf{93.9}  \\
                                  & FE                                              & 87.6                  & 78.3                & 91.6           \\
                                  & PB \cite{piggyback}                             & 89.4                  & 83.5                & 89.6           \\
                                  & BAT \cite{quantized}                            & \textbf{92.9}         & \textbf{83.7}       & 93.5           \\
                                  & RS  \cite{rebuffi_1}                            & 90.9                  & 83.6                & 93.7           \\
                                  & RP \cite{rebuffi_2}                             & 91.3                  & \textbf{83.7}       & 93.8           \\ \hline
\multirow{6}{*}{\textbf{LineMOD}} & FT                                              & \textbf{96.7}         & \textbf{87.0}       & \textbf{96.9}          \\
                                  & FE                                              & 13.9                  & 7.6                 & 14.8          \\
                                  & PB \cite{piggyback}                             & 95.9                  & 83.2                & 96.6          \\
                                  & BAT \cite{quantized}                            & 95.0                  & \textbf{87.0}       & 95.2          \\
                                  & RS  \cite{rebuffi_1}                            & 89.7                  & 79.8                & 93.8          \\
                                  & RP \cite{rebuffi_2}                             & 89.9                  & 76.9                & 92.1          \\ \hline
\multirow{6}{*}{\textbf{NYU}}     & FT                                              & 67.5                  & 59.2                & 68.4          \\
                                  & FE                                              & 57.9                  & 43.1                & 60.2          \\
                                  & PB \cite{piggyback}                             & \textbf{68.4}         & 56.6                & 66.7          \\
                                  & BAT \cite{quantized}                            & 68.1                  & 57.3                & 68.1          \\
                                  & RS  \cite{rebuffi_1}                            & 67.1                  & \textbf{61.2}       & \textbf{70.9} \\
                                  & RP \cite{rebuffi_2}                             & 68.3                  & 57.3                & 67.5         \\\hline
\end{tabular}}
\end{table}


==> tables_old.tex <==
\begin{table*}[t]
\caption{Results in term of accuracy for the RGB-D Triathlon challenge in the RGB setting. The best method is bold, the second best is underlined.}
\label{tab:scoreRGB}
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l|c|cc|cc|cc}
Metric            & Par. & AvgA           & AAPR           & Deca            & RevD                    & \textbf{Linear}  \\ \hline     %& LiWP                                 
Fine-tuning                   & 3    & {\ul 85.0}    & 28.3          & \textbf{750} & 161           & 0             \\                  %& 1000                                 
Feature extractor             & 1    & 53.1          & 53.1          & 229          & 229           & 0             \\                  %& 0                                    
Piggyback \cite{piggyback}    & 1.10 & 84.5          & {\ul 77.2}    & 577          & {\ul 472}     & {\ul 826}     \\                  %& 880                                    
BAT \cite{quantized}          & 1.10 & \textbf{85.3} & \textbf{77.9} & {\ul 692}    & \textbf{566}  & \textbf{1159} \\                  %& \textbf{1235}                          
R.a. series  \cite{rebuffi_1} & 1.47 & 82.6          & 56.2          & 500          & 239           & 706           \\                  %& 969                                    
R.a. parallel \cite{rebuffi_2}& 1.38 & 83.2          & 60.5          & 541          & 288           & 819                               %& {\ul 1053}       
\end{tabular}
}
\end{table*}

\begin{table*}[t]
\caption{Results in term of accuracy for the RGB-D Triathlon challenge in the D setting. The best method is bold, the second best is underlined.}
\label{tab:scoreD}
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l|c|cc|cc|cc}
Metric            & Par. & AvgA           & AAPR           & Deca            & RevD                      & \textbf{Linear} \\ \hline    %& LiWP                          
Fine-tuning                   & 3    & \textbf{76.5} & 25.5           & \textbf{750}    & 161            & 0               \\           %& {\ul 1000}            
Feature extractor             & 1    & 43.0          & 43.0           & 212             & 212            & 0               \\           %& 0                     
Piggyback \cite{piggyback}    & 1.10 & 74.4          & {\ul 67.9}     & 598             & {\ul 489}      & {\ul 881}    \\              %& 939               
BAT \cite{quantized}          & 1.10 & {\ul 76.0}    & \textbf{69.4}  & {\ul 740}       & \textbf{606}   & \textbf{927} \\              %& 988               
R.a. series  \cite{rebuffi_1} & 1.47 & 74.8          & 50.9           & 581             & 278            & 748             \\           %& \textbf{1026}         
R.a. parallel \cite{rebuffi_2}& 1.38 & 72.6          & 52.8           & 501             & 267            & 732                          %& 942               
\end{tabular}%
}
\end{table*}


\begin{table*}[t]
\caption{Results in term of accuracy for the RGB-D Triathlon challenge in the RGB+D setting. The best method is bold, the second best is underlined.}
\label{tab:scoreRGBD}
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l|c|cc|cc|cc}

Metric                         & Par.   & AvgA          & AAPR          & Deca          & RevD          & \textbf{Linear} \\ \hline   %& LiWP            
Fine-tuning                    & 3      & \textbf{86.4} & 28.8          & \textbf{750}  & 161           & 0    \\                     %& {\ul 1000}      
Feature extractor              & 1      & 55.5          & 55.5          & 23            & 236           & 0    \\                     %& 0               
Piggyback \cite{piggyback}     & 1.10   & 84.2          & {\ul 76.8}    & 450           & {\ul 368}     & 543    \\                   %& 578                 
BAT \cite{quantized}           & 1.10   & 85.6          & \textbf{78.1} & 514           & \textbf{420}  & \textbf{862} \\             %& 919                             
R.a. series  \cite{rebuffi_1}  & 1.47   & \textbf{86.1} & 58.6          & {\ul 523}     & 250           & {\ul 770} \\                %& \textbf{1057}                   
R.a. parallel \cite{rebuffi_2} & 1.38   & 84.5          & 61.4          & 481           & 256           & 727                         %& 935                     
\end{tabular}%
}
\end{table*}

